Beyond task success: A closer look at jointly learning to see, ask, and GuessWhat

We propose a grounded dialogue state encoder which addresses a foundational issue on how to integrate visual grounding with dialogue system components. As a test-bed, we focus on the GuessWhat?! game, a two-player game where the goal is to identify an object in a complex visual scene by asking a sequence of yes/no questions. Our visually-grounded encoder leverages synergies between guessing and asking questions, as it is trained jointly using multi-task learning. We further enrich our model via a cooperative learning regime. We show that the introduction of both the joint architecture and cooperative learning lead to accuracy improvements over the baseline system. We compare our approach to an alternative system which extends the baseline with reinforcement learning. Our in-depth analysis shows that the linguistic skills of the two models differ dramatically, despite approaching comparable performance levels. This points at the importance of analyzing the linguistic output of competing systems beyond numeric comparison solely based on task success.

==> qualitative_analysis.tex <==

\subsection{Qualitative Analysis of Dialogues}

\rb{There is no ref. in the text above to the figure with the dialogue
example}

\begin{figure}\centering
\includegraphics[width=7.9cm]{images/example1_target_box.pdf}
\caption{Example of a successful game played by our CL model. The model guesses the target correctly, although some of the questions and answers are difficult to interpret with respect to the image.
\bp{update fig - do we have a comparative one, CL vs RL? (one run)}
}
\label{fig:example}
\end{figure}









\cut{%
\subsection{Quality of the dialogues}

After having made all these quantitative comparisons of the models, it
is interesting to look at the quality of their dialogues. Quite
surprisingly, the cooperative model seems to  have acquired
sophisticated linguistic skills, for instance it is able to use
anaphora, like in the following exchange ``is it the one in the
middle with the white shirt and black pants? $<$yes$>$; is it the one to
the left of him, black shorts, and pants?''. Moreover it uses non-trivial spatial questions like ``is it the person that is closest to
the left side of the photo ?''. As we said before, differently from the models, which almost always start with an {\sc
  entity} question, We conjecture this could be due to the renown
fact that neural networks are good at identifying objects and have still
difficulties in distinguishing
attribute. \rb{Following~\cite{shek:askn18} we have checked the
  presence of repetitions in the dialogue. Of the games played by the
  Baseline 98\% contains at least one question repeated and  72.26 of
  the 
  games contains at least 1 repetition between consecutive questions. The games
  played by our model contains much less repetition: 66.23 and 59.97,
  SL and CL, respectively. And the number decreases even further if
  we consider the consecutive repetitions: 42.83 (SL) and 44.44 (CL).
  See the Supplementary Material for more details.}
\cut{
Manual inspection of the generated dialogues shows that the Questioner models often asks the same question more than once over the course of a game --- what should have been established as known information seems to have been forgotten, which renders the dialogue unnatural. We analyse the generated dialogues in terms of the amount of repeated questions they contain. 
\rf{Cite COLING paper \cite{shek:askn18} for this kind of analysis, if
  accepted}
\rb{The nr of repetitions suc vs unsucc.}
\rf{Should we consider only verbatim repetitions of questions classified as {\sc entity}?}
\rf{Report percentage of repeated questions for BL, SL and CL.}
}



\cut{ 
Image Id : COCO_train2014_000000271689.jpg
< Ours-CL > : <start> is it a person ? <yes> is it the one in front ?
<yes> is the person wearing a red shirt ? <yes> is the person in the
foreground ? <yes> is the person in the middle ? <yes> is it the one
with the white shirt ? <yes> is it the one in the front wearing white
? <yes> is it the one on the far right ? <no> is it the one in the
middle with the white shirt and black pants ? <yes> is it the one to
the left of him , black shorts , and pants ? <yes> < Game Status :
success>
} 



\cut{
Game ID : 3466> <
Image Id : COCO_train2014_000000521981.jpg

< GL > : Is it a person? <Yes> Is it female? <no> Does he have skis or ski poles? <no> Is he on the far left? <Yes> <<<<< Target Obj : person>>>>>

< BL > : <start> is it a person ? <yes> is it in the foreground ? <no>
is it in the foreground ? <no> is it in the foreground ? <no> is it in
the background ? <yes> is it in the foreground ? <no> is it in the
background ? <yes> is it in the background ? <yes> is it in the right
side of the picture ? <no> is it in the middle ? <no> <<<<< Guessed
Obj : person>>>>> < Game Status : failure>

< Ours-SL > : <start> is it a person ? <yes> is it the person on the
far left ? <yes> is it the whole person ? <yes> is it the person on
the far left ? <yes> is it the whole person ? <yes> is it the person
on the left in the white ? <yes> is it the person that is closest to
the left side of the photo ? <yes> is it the whole person ? <yes> is
it the person closest to the left side of the photo ? <yes> is it all
of the human that we can see in the picture ? <yes>< Game Status :
success>
}

}



\cut{

Image Id : COCO_train2014_000000075369.jpg

< GL > : Is it red? <no> Is it white? <Yes> is it in the foreground? <Yes> Is it on the right? <Yes> <<<<< Target Obj : sandwich>>>>>

< BL > : <start> is it food ? <yes> is it on the plate ? <yes> is it on the left ? <no> is it the hot dog ? <yes> is it on the left ? <no> is it the one on the right ? <yes> is it the one on the left ? <no> is it the one on the right ? <yes> is it the one on the left ? <no> is it the one on the right ? <yes> <<<<< Guessed Obj : sandwich>>>>> < Game Status : success>

< Ours-SL > : <start> is it food ? <yes> is it a hot dog ? <yes> is it the one on the left ? <no> is it the one on the right ? <yes> is it the entire hotdog ? <yes> is it the one on the right ? <yes> is it the whole one ? <yes> is it on top ? <yes> is it the one on top ? <yes> is it the whole sandwich ? <yes>< Game Status : success>

< Ours-CL > : <start> is it food ? <yes> is it in the first plate
closest to the camera ? <yes> is it in the middle of the picture ?
<yes> is it the one closest to the bottom of the picture ? <yes> does
it have something to do with the bun in the bun ? <yes> is it all the
food in the middle of the picture ? <yes> is it the one closest to the
right side of the picture ? <yes> so its the one that is at the very
bottom of the picture ? <yes> is it the entire portion of the fries ?
<yes> second from the right ? <yes> < Game Status : success>
}


\cut{The constraint of having a fixed number of questions forces the models
to ask uncessary questions. Following~\cite{shek:askn18}, in the next
section we extend the joint end-to-end learning approch by including
also a decider module.
}




